Learning Camera Localization via Dense Scene Matching

Camera localization aims to estimate 6 DoF camera poses from RGB images. Traditional methods detect and match interest points between a query image and a pre-built 3D model. Recent learning-based approaches encode scene structures into a specific convolutional neural network (CNN) and thus are able to predict dense coordinates from RGB images. However, most of them require re-training or re-adaption for a new scene and have difficulties in handling large-scale scenes due to limited network capacity. We present a new method for scene agnostic camera localization using dense scene matching (DSM), where a cost volume is constructed between a query image and a scene. The cost volume and the corresponding coordinates are processed by a CNN to predict dense coordinates. Camera poses can then be solved by PnP algorithms. In addition, our method can be extended to temporal domain, which leads to extra performance boost during testing time. Our scene-agnostic approach achieves comparable accuracy as the existing scene-specific approaches, such as KFNet, on the 7scenes and Cambridge benchmark. This approach also remarkably outperforms state-of-the-art scene-agnostic dense coordinate regression network SANet. The Code is available at https://github.com/Tangshitao/Dense-Scene-Matching.

==> 3_2_pyramid2__depracated_.tex <==
\subsection{Feature Pyramid and coordinate preprocessing }\label{sec::feature_pyramid}
Given one query image $\mathbf{Q}_t$ at time $t$ and multiple reference scene images $\{\mathbf{S}_i| i = 1,...,n\}$, we generate a $L$-level pyramid of feature maps $\{\mathbf{F}^l| l = 1,...,L\}$ for each of them by ResNet50-FPN~\cite{lin2017feature}. We denote the query feature maps as $\mathbf{F}_{q}^l$ and the scene feature maps as $\mathbf{F}_{s}^l$. 
%The feature vectors in $\mathbf{F}_{q}^l$ are referred as $\mathbf{f}_{q}^{l}$, and those in $\mathbf{F}_{s}^l$ are $\mathbf{f}_{s}^{l}$.
%Note that the spatial size of $\mathbf{F}^l$ is downsampled from $\mathbf{F}^{l-1}$ by a factor of 2. 
The spatial size of feature maps at level $l$ is $H^l\times W^l$.

The coordinates of scene images form coordinate collections. We also build $L$-level coordinate collections, corresponding to $L$-level feature pyramid. The coordinates in $l^{th}$ collections are averaged pooled from the ones in ${l-1}^{th}$ collections with respect to scene images by a factor of 2. In order to deal with scenes at different scales, we transform the 3D scene coordinates to a local coordinate system, where the coordinates are normalized to zero-mean and unit standard deviation at all $x, y, z$ channels. Each coordinate is associated with a fused feature vector, which is obtained by averaging corresponding feature vectors in different scene feature maps $\mathbf{F}_{s}^l$. 

%with the mean coordinate at origin and normalize by subtracting their mean value for  respectively and divided by a single standard deviation value computed for all $x, y, z$ channels.
% To facilitate the network training, we obtain the relative coordinates by subtracting all the coordinates in the cost-coordinate volume by the upsampled coordinates from the previous level.

We estimate the coordinate map in a coarse-to-fine manner.
%, we further denote the output coordinate map at each level as $\mathbf{D}^l$. 
After initializing the coarsest level, the coordinate map $\mathbf{\hat{D}}^{l}$ at level $l$ is initialized by upsampling from $\mathbf{D}^{l+1}$.

==> 3_3_dense_matching2__depracated_.tex <==
\subsection{Dense Scene Matching}\label{sec:corr}
The overview of the DSM module is shown in Fig.~\ref{fig:CRM}.
At a specific level $l$, the input of DSM module includes: 1) query image feature maps $\mathbf{F}_{q}^l$; 2) scene image feature maps $\mathbf{F}_{s}^l$ and corresponding scene coordinate maps $\mathbf{M}^l$; 3) initial coordinate maps $\mathbf{\hat{D}}^{l}$ upsampled from $\mathbf{D}^{l+1}$.
% \ping{Some introduction/motivation is needed here. Talking about why a cost volume is needed.}
The DSM module predicts the coordinate map $\mathbf{D}^{l}$ with more details from the initial $\mathbf{\hat{D}}^{l}$.
Specifically, DSM consists of two steps, namely cost volume construction and coordinate regression.
It first constructs a cost volume which measures the correlations between 2D query pixels and scene points (with known coordinates). 
It then regresses a dense coordinate map of the query image from the cost volume.
%The cost volume guides the interpolation of the coordinate map. 


\subsubsection{Cost Volume Construction}\label{cost_vol}
This section explains the details of cost volume construction, which involves two processes, namely the scene correlation and temporal correlation.
The scene correlation measure similarity between query image pixels and scene points, while the temporal correlation measure the similarity between query image pixels from two neighboring frames in the query video clip.
Our network only uses scene correlation in training, and fuses both correlations at testing time.

%from both query-scene and temporal correlations.
%The definition of scene correlation and temporal correlation is given below followed by the details of cost volume construction. 
%Fig.\ref{fig:CRM} visualizes the concept of scene correlation, temporal correlation and correlation fusion.

% \vspace{-0.5cm}
\paragraph{Scene correlation.} 
As shown in Fig.\ref{fig:Corr}, for an pixel $\mathbf{q}$ in the query feature map $\mathbf{F}_{q}^{l}$, we obtain its 3D coordinate from the initial coordinate map $\mathbf{\hat{D}}^{l}$. After that, we can project this 3D point to the reference scene image feature map $\mathbf{F}_{s}^l$. Suppose the projected position is $\mathbf{p}$. We consider a $d\times d$ search window centered at $\mathbf{p}$ and compute the cosine similarity between the feature vector at $\mathbf{q}$ and those feature vectors for the pixels within the search window. In this way, we obtain a correlation vector of size $d*d$ at the query pixel at $\mathbf{q}$. Given $N$ reference scene images, we obtain a $N*d*d$ scene correlations per pixel, which aggregate to a $H^l\times W^l \times (N*d*d)$ tensor, named correlation matrix. For the coarsest level, we compute the correlation between each query pixel and the whole scene feature maps since its initial depth is unknown.

%we obtain $N\times H^L\times W^L$ scene correlations in the coarsest level and where $H^L$ and $W^L$ is the height and width of the coarsest feature maps,  and $N$ is the number of retrieved scene images. 

%Consequently, for each query pixel, 
% \vspace{-0.5cm}
\paragraph{Temporal correlation.} 
If the query input is a video sequence, we can leverage the result at the previous frame and the  correlation between neighboring video frames to enhance the result. 
Basically, if the camera pose is known, we can project a scene point $\mathbf{p}$ into the query video frame $\mathbf{Q}_{t-1}$ at $\mathbf{q}'$. Then the correlation between $\mathbf{p}$ and the query pixel $\mathbf{q}$ in video frame $\mathbf{Q}_{t}$ can be evaluated by the correlation between the two query pixels $\mathbf{q}'$ and $\mathbf{q}$.
%correlation between the feature maps of consecutive video frames. 


Specifically, we project all scene points in the $d \times d$ search window to the query image $\mathbf{Q}_{t-1}$ according to the camera pose at $t-1$.
Subsequently, we can compute the correlation between the feature vector at a query pixel in $\mathbf{Q}_{t}$ and the feature vectors of these projected pixels in $\mathbf{Q}_{t-1}$. In this way, for each query pixel, we also obtain a correlation vector of size $N*d*d$ by temporal correlation.

%for each pixel of query image $\mathbf{Q}_{t}$ at time $t$, we first project all its corresponding scene coordinates in coordinate map $\mathbf{M}^l$ within the searching space to the query image $\mathbf{Q}_{t-1}$ at time $t-1$. 
%If the estimated camera pose of $\mathbf{Q}_{t-1}$ is accurate enough, this projection should lead to the true corresponding point of $\mathbf{f}_{q,t}^l$ in the previous query image. 


% \vspace{-0.5cm}
\paragraph{Correlation fusion.} 
The final correlation score between a query pixel and a scene point is then computed from the scene correlation and temporal correlation by the following equation,
\begin{equation}
\label{equ:fusion}
    Corr=\alpha Corr_s+(1-\alpha) Corr_t,
\end{equation}
where $Corr_s$ stands for scene correlations and $Corr_t$ is temporal correlations. The parameter $\alpha$ balances $Corr_s$ and $Corr_t$. 
%We first only use scene correlations to estimate confidence scores, as illustrated above. 
The hyper-parameter $\alpha$ is derived from the confidence score by $\alpha=\beta s$, where $\beta$ is set to 0.9 empirically and $s$ is the confidence score, which will be introduced shortly. Note that the fusion in \equref{equ:fusion} is applied to each of the $N$ reference scene images. At the end of this fusion, we obtain a fused correlation matrix of size $H^l\times W^l \times (N*d*d)$.

%and will be introduced shortly.
%estimated as the average confidence score over all pixels in a query image.
% \vspace{-0.5cm}
\paragraph{Cost volume.}
The size of correlation matrix varies according to $N$, which might change from query image to query image. To address this problem, we construct a cost volume by sorting the correlation values and selecting the top-$K$ ($K=32$ in our implementation) scene coordinates. Although the sorting operation is not differentiable, the gradients can still be passed by the correlation values in the backward propagation during training. Intuitively, a higher correlation score means more accurate match between query pixels and scene points. 

%Assuming the spatial size of the query feature map $\mathbf{F}_q^l$ is $H^l \times W^l$, we can then construct a volume with a size of $H^l \times W^l \times K$. And the cost volume size is fixed at
After sorting, we obtain a cost volume of size $H^l \times W^l \times K$. We further concatenate this cost volume with the 3D scene coordinates of corresponding scene points to form a $H \times W \times 4K$ (1 for correlation and 3 for scene coordinates) cost-coordinate volume. This cost-coordinate volume is then processed by CNN to produce a dense coordinate map.


% \subsubsection{Temporal fusion}
% \paragraph{Temporal correlation.} 
% \ping{this paragraph is very dense and difficult to follow. A figure might be necessary}
% If the query input is a video sequence, we can further leverage the correlation between the feature maps of consecutive video frames. 
% %Following the projection in computing scene correlations, 
% Specifically, for each feature vector $\mathbf{f}_{q,t}^l$, we project the scene coordinates inside its $d\times d$ \textit{searching window} to the previous query image $\mathbf{Q}_{t-1}$ at time $t-1$ with its estimated pose.
% If the scene coordinate is correct, this projection should lead to the true corresponding point of $\mathbf{f}_{q,t}^l$ in the previous query image. 
% Therefore, we can evaluate the correlation between $\mathbf{f}_{q,t}^l$ and the feature at the projected pixel, i.e. $\mathbf{f}_{q,{t-1}}^l$, to evaluate the quality of the scene coordinates in the $d\times d$ \textit{searching window}. 

%Thus we obtain the feature correspondences between the feature maps $\mathbf{F}_{q,t}^l$ and $\mathbf{F}_{q,t-1}^l$. Finally, the temporal correlation is calculated as cosine similarity of and . 

% We will fuse the scene correlation with temporal correlation to further improve the accuracy of query-scene correspondences


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/corr_fig.pdf}
    \caption{Demonstration of correlation fusion process. For a specific pixel $\mathbf{q}$ in $\mathbf{F}_{q,t}^l$, we obtain its scene correlation by projecting its corresponding 3D coordinate predicted in $\mathbf{\hat{D}}^l$ to a searching space in retrieved $N$ scene feature maps $\mathbf{F}_s^l$. Temporal correlation is obtained by projecting the scene coordinates within the searching space in $\mathbf{M}^l$ to $\mathbf{F}_{q,t-1}^l$. Finally, a $N \times d \times d$ correlation vector is formed for each query pixel.}
    \label{fig:Corr}
\end{figure}
\subsubsection{Confidence Estimation}
In order to fuse the temporal correlations and scene correlations, we predict a confidence value $s$ as the weighting parameter, as discussed in Sec. \ref{cost_vol}. We use a network denoted as $Net_{conf}$, consisting of $1\times 1$ convolutional layers, to take the cost-coordinate volume as input. 
$Net_{conf}$ then predicts an uncertainty score for each pixel, which measures how accurate the coordinate prediction is. During training, we treat it as a classification problem. If the reprojection error of all top-K coordinates with respect to ground truth is larger than some threshold (1 pixel in implementation), we classify it as an uncertain pixel and $Net_{conf}$ predicts whether it is a uncertain pixel by outputting an uncertainty score. Cross entropy loss is used during training. The final confidence $s$ is estimated by averaging all the confidence scores, which is computed by ($1-uncertainty$), over all pixels. $Net_{conf}$ is designed to be light-weight, which enables fast inference for video sequence. 
%The detailed architecture of $Net_A$ will be introduced in the supplementary material.


\subsubsection{Coordinate Regression}\label{CRM}
Apart from confidence scores, ${Net}_{conf}$ also produces a coordinate feature map encoding the coordinate information. Then we use another network namely ${Net}_{coords}$, consisting of $3\times 3$ convolutional layers, to estimate the final scene coordinate map from the coordinate feature map, query image features, and initial coordinate map by up-sampling from a caorser resolution.
The ${Net}_{conf}$ and ${Net}_{coords}$ use different parameters and we present their architectures in the supplementary material. 
